STAR: Semantic-Criticality Tiered Allocation of Radio Resources via Zero-Shot Learning

In remote inference, edge devices transmit high-resolution images over wireless links to a receiver, where an artificial intelligence (AI) model answers task-specific questions about these images to enable reliable decisions. These answers are often determined by a small set of task-causal pixels, such as those of text, whose corruption changes the answer, so these pixels must be delivered with high fidelity. Conventional transmission protects every pixel equally, so it either consumes many resource elements (REs) or corrupts these regions at low signal-to-noise ratio (SNR). To overcome these limitations, in this paper, a zero-shot, domain-agnostic framework, termed semantic-criticality tiered allocation of resources (STAR), is proposed. In particular, a per-pixel semantic-criticality indicator (SCI) is derived from the attention of a frozen vision-language model, so new tasks and domains are handled by changing only the prompt, without retraining. The resulting task causality-aware resource allocation problem over protection tiers is solved exactly by a threshold rule on the SCI, realized by a coded tier for the task-causal pixels and an uncoded, downsampled base layer for the full image. Simulations over a 5G New Radio link demonstrate that STAR attains a semantic accuracy of at least 0.98 for $E_s/N_0 \geq -4$ dB and, at comparable semantic reliability, reduces the REs of robust coded transmission by 59.5% and 91.5% on factory- and vehicle-monitoring datasets, respectively, the latter without any change to the models. Although a deep joint source-channel coding baseline uses fewer REs at comparable semantic accuracy, it must be retrained with labeled data for every new task or domain.

==> defines.tex <==
%\newtheorem{lemma}{Lemma}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\st}{\scriptstyle}
\newcommand{\sst}{\scriptscriptstyle}
\newcommand{\etal}{{\it  et al.\ }}
\newcommand{\lb}{\left(}
\newcommand{\rb}{\right)}
\newcommand{\lsb}{\left[}
\newcommand{\rsb}{\right]}
\newcommand{\la}{\left\{ }
\newcommand{\ra}{\right\} }
\newcommand{\lac}{\left\{}
\newcommand{\rac}{\right\} }
\newcommand{\lan}{\left\langle }
\newcommand{\ran}{\right\rangle }
\newcommand{\lbg}{\left\lceil}
\newcommand{\rbg}{\right\rceil}
\newcommand{\lbf}{\left\lfloor}
\newcommand{\rbf}{\right\rfloor}
\newcommand{\defi}{\stackrel{\bigtriangleup}{=}}
\newcommand{\m}{{\!\, -\!\,}}
\newcommand{\p}{{\!\, +\!\,}}
\newcommand{\T}{H}
%\newcommand{\tc}{t}
\newcommand{\tT}{T}
\newcommand{\tcc}{*}
\newcommand{\w}{w}
\newcommand{\z}{{\it z}}	% z-transform
\newcommand{\eps}{\epsilon}
\newcommand{\at}{@@}
\newcommand{\dprod}{\displaystyle\prod}

% TEXT AND MATH STYLES
%\newcommand{\bmf}[1]{\mbox{\boldmath ${#1}$}}
%\newcommand{\bmfscript}[1]{\mbox{\scriptsize{\boldmath $\displaystyle{#1}$}}}
\newtheorem{Thm}{\bf Theorem}
\newcommand{\mbf}[1]{\mbox{\boldmath ${#1}$}}
\newcommand{\mbfscript}[1]{\mbox{\scriptsize{\boldmath $\displaystyle{#1}$}}}
% BOLD CAPITALS for maths
\newcommand{\bdmA}{\mbox{\boldmath $A$}}
\newcommand{\bdmB}{\mbox{\boldmath $B$}}
\newcommand{\bdmC}{\mbox{\boldmath $C$}}
\newcommand{\bdmD}{\mbox{\boldmath $D$}}
\newcommand{\bdmE}{\mbox{\boldmath $E$}}
\newcommand{\bdmF}{\mbox{\boldmath $F$}}
\newcommand{\bdmG}{\mbox{\boldmath $G$}}
\newcommand{\bdmH}{\mbox{\boldmath $H$}}
\newcommand{\bdmI}{\mbox{\boldmath $I$}}
\newcommand{\bdmJ}{\mbox{\boldmath $J$}}
\newcommand{\bdmK}{\mbox{\boldmath $K$}}
\newcommand{\bdmL}{\mbox{\boldmath $L$}}
\newcommand{\bdmM}{\mbox{\boldmath $M$}}
\newcommand{\bdmN}{\mbox{\boldmath $N$}}
\newcommand{\bdmO}{\mbox{\boldmath $O$}}
\newcommand{\bdmP}{\mbox{\boldmath $P$}}
\newcommand{\bdmQ}{\mbox{\boldmath $Q$}}
\newcommand{\bdmR}{\mbox{\boldmath $R$}}
\newcommand{\bdmS}{\mbox{\boldmath $S$}}
\newcommand{\bdmT}{\mbox{\boldmath $T$}}
\newcommand{\bdmU}{\mbox{\boldmath $U$}}
\newcommand{\bdmV}{\mbox{\boldmath $V$}}
\newcommand{\bdmW}{\mbox{\boldmath $W$}}
\newcommand{\bdmX}{\mbox{\boldmath $X$}}
\newcommand{\bdmY}{\mbox{\boldmath $Y$}}
\newcommand{\bdmZ}{\mbox{\boldmath $Z$}}


% BOLD small letters for math

\newcommand{\bdma}{\mbox{\boldmath $a$}}
\newcommand{\bdmb}{\mbox{\boldmath $b$}}
\newcommand{\bdmc}{\mbox{\boldmath $c$}}
\newcommand{\bdmd}{\mbox{\boldmath $d$}}
\newcommand{\bdme}{\mbox{\boldmath $e$}}
\newcommand{\bdmf}{\mbox{\boldmath $f$}}
\newcommand{\bdmg}{\mbox{\boldmath $g$}}
\newcommand{\bdmh}{\mbox{\boldmath $h$}}
\newcommand{\bdmi}{\mbox{\boldmath $i$}}
\newcommand{\bdmj}{\mbox{\boldmath $j$}}
\newcommand{\bdmk}{\mbox{\boldmath $k$}}
\newcommand{\bdml}{\mbox{\boldmath $l$}}
\newcommand{\bdmm}{\mbox{\boldmath $m$}}
\newcommand{\bdmn}{\mbox{\boldmath $n$}}
\newcommand{\bdmo}{\mbox{\boldmath $o$}}
\newcommand{\bdmp}{\mbox{\boldmath $p$}}
\newcommand{\bdmq}{\mbox{\boldmath $q$}}
\newcommand{\bdmr}{\mbox{\boldmath $r$}}
\newcommand{\bdms}{\mbox{\boldmath $s$}}
\newcommand{\bdmt}{\mbox{\boldmath $t$}}
\newcommand{\bdmu}{\mbox{\boldmath $u$}}
\newcommand{\bdmv}{\mbox{\boldmath $v$}}
\newcommand{\bdmw}{\mbox{\boldmath $w$}}
\newcommand{\bdmx}{\mbox{\boldmath $x$}}
\newcommand{\bdmy}{\mbox{\boldmath $y$}}
\newcommand{\bdmz}{\mbox{\boldmath $z$}}

% SERIF CAPITALS for maths

\newcommand{\srfA}{\mbox{$\mathsf A$}}
\newcommand{\srfB}{\mbox{$\mathsf B$}}
\newcommand{\srfC}{\mbox{$\mathsf C$}}
\newcommand{\srfD}{\mbox{$\mathsf D$}}
\newcommand{\srfE}{\mbox{$\mathsf E$}}
\newcommand{\srfF}{\mbox{$\mathsf F$}}
\newcommand{\srfG}{\mbox{$\mathsf G$}}
\newcommand{\srfH}{\mbox{$\mathsf H$}}
\newcommand{\srfI}{\mbox{$\mathsf I$}}
\newcommand{\srfJ}{\mbox{$\mathsf J$}}
\newcommand{\srfK}{\mbox{$\mathsf K$}}
\newcommand{\srfL}{\mbox{$\mathsf L$}}
\newcommand{\srfM}{\mbox{$\mathsf M$}}
\newcommand{\srfN}{\mbox{$\mathsf N$}}
\newcommand{\srfO}{\mbox{$\mathsf O$}}
\newcommand{\srfP}{\mbox{$\mathsf P$}}
\newcommand{\srfQ}{\mbox{$\mathsf Q$}}
\newcommand{\srfR}{\mbox{$\mathsf R$}}
\newcommand{\srfS}{\mbox{$\mathsf S$}}
\newcommand{\srfT}{\mbox{$\mathsf T$}}
\newcommand{\srfU}{\mbox{$\mathsf U$}}
\newcommand{\srfV}{\mbox{$\mathsf V$}}
\newcommand{\srfW}{\mbox{$\mathsf W$}}
\newcommand{\srfX}{\mbox{$\mathsf X$}}
\newcommand{\srfY}{\mbox{$\mathsf Y$}}
\newcommand{\srfZ}{\mbox{$\mathsf Z$}}

% SERIF small letters for math

\newcommand{\srfa}{\mbox{$\mathsf a$}}
\newcommand{\srfb}{\mbox{$\mathsf b$}}
\newcommand{\srfc}{\mbox{$\mathsf c$}}
\newcommand{\srfd}{\mbox{$\mathsf d$}}
\newcommand{\srfe}{\mbox{$\mathsf e$}}
\newcommand{\srff}{\mbox{$\mathsf f$}}
\newcommand{\srfg}{\mbox{$\mathsf g$}}
\newcommand{\srfh}{\mbox{$\mathsf h$}}
\newcommand{\srfi}{\mbox{$\mathsf i$}}
\newcommand{\srfj}{\mbox{$\mathsf j$}}
\newcommand{\srfk}{\mbox{$\mathsf k$}}
\newcommand{\srfl}{\mbox{$\mathsf l$}}
\newcommand{\srfm}{\mbox{$\mathsf m$}}
\newcommand{\srfn}{\mbox{$\mathsf n$}}
\newcommand{\srfo}{\mbox{$\mathsf o$}}
\newcommand{\srfp}{\mbox{$\mathsf p$}}
\newcommand{\srfq}{\mbox{$\mathsf q$}}
\newcommand{\srfr}{\mbox{$\mathsf r$}}
\newcommand{\srfs}{\mbox{$\mathsf s$}}
\newcommand{\srft}{\mbox{$\mathsf t$}}
\newcommand{\srfu}{\mbox{$\mathsf u$}}
\newcommand{\srfv}{\mbox{$\mathsf v$}}
\newcommand{\srfw}{\mbox{$\mathsf w$}}
\newcommand{\srfx}{\mbox{$\mathsf x$}}
\newcommand{\srfy}{\mbox{$\mathsf y$}}
\newcommand{\srfz}{\mbox{$\mathsf z$}}

\newcommand{\oneb}{\mbox{\boldmath $1$}}
\newcommand{\zerb}{\mbox{\boldmath $0$}}

\newcommand{\Us}{\mbox{$\mathcal U$}}
\newcommand{\Vs}{\mbox{$\mathcal V$}}

% CAPITAL VERTICAL FONTS

\newcommand{\bdSA}{\mbox{\bf A}}
\newcommand{\bdSB}{\mbox{\bf B}}
\newcommand{\bdSC}{\mbox{\bf C}}
\newcommand{\bdSD}{\mbox{\bf D}}
\newcommand{\bdSE}{\mbox{\bf E}}
\newcommand{\bdSF}{\mbox{\bf F}}
\newcommand{\bdSG}{\mbox{\bf G}}
\newcommand{\bdSH}{\mbox{\bf H}}
\newcommand{\bdSI}{\mbox{\bf I}}
\newcommand{\bdSJ}{\mbox{\bf J}}
\newcommand{\bdSK}{\mbox{\bf K}}
\newcommand{\bdSL}{\mbox{\bf L}}
\newcommand{\bdSM}{\mbox{\bf M}}
\newcommand{\bdSN}{\mbox{\bf N}}
\newcommand{\bdSO}{\mbox{\bf O}}
\newcommand{\bdSP}{\mbox{\bf P}}
\newcommand{\bdSQ}{\mbox{\bf Q}}
\newcommand{\bdSR}{\mbox{\bf R}}
\newcommand{\bdSS}{\mbox{\bf S}}
\newcommand{\bdST}{\mbox{\bf T}}
\newcommand{\bdSU}{\mbox{\bf U}}
\newcommand{\bdSV}{\mbox{\bf V}}
\newcommand{\bdSW}{\mbox{\bf W}}
\newcommand{\bdSX}{\mbox{\bf X}}
\newcommand{\bdSY}{\mbox{\bf Y}}
\newcommand{\bdSZ}{\mbox{\bf Z}}


\newcommand{\bdSa}{\mbox{\bf a}}
\newcommand{\bdSb}{\mbox{\bf b}}
\newcommand{\bdSc}{\mbox{\bf c}}
\newcommand{\bdSd}{\mbox{\bf d}}
\newcommand{\bdSe}{\mbox{\bf e}}
\newcommand{\bdSf}{\mbox{\bf f}}
\newcommand{\bdSg}{\mbox{\bf g}}
\newcommand{\bdSh}{\mbox{\bf h}}
\newcommand{\bdSi}{\mbox{\bf i}}
\newcommand{\bdSj}{\mbox{\bf j}}
\newcommand{\bdSk}{\mbox{\bf k}}
\newcommand{\bdSl}{\mbox{\bf l}}
\newcommand{\bdSm}{\mbox{\bf m}}
\newcommand{\bdSn}{\mbox{\bf n}}
\newcommand{\bdSo}{\mbox{\bf o}}
\newcommand{\bdSp}{\mbox{\bf p}}
\newcommand{\bdSq}{\mbox{\bf q}}
\newcommand{\bdSr}{\mbox{\bf r}}
\newcommand{\bdSs}{\mbox{\bf s}}
\newcommand{\bdSt}{\mbox{\bf t}}
\newcommand{\bdSu}{\mbox{\bf u}}
\newcommand{\bdSv}{\mbox{\bf v}}
\newcommand{\bdSw}{\mbox{\bf w}}
\newcommand{\bdSx}{\mbox{\bf x}}
\newcommand{\bdSy}{\mbox{\bf y}}
\newcommand{\bdSz}{\mbox{\bf z}}
\newcommand{\mZ}{\mathcal{Z}}

\newcommand{\cA}{{\mathcal A}}
\newcommand{\ca}{{\mathcal a}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cb}{{\mathcal b}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cc}{{\mathcal c}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cd}{{\mathcal d}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\ce}{{\mathcal e}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cf}{{\mathcal f}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cg}{{\mathcal g}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\ch}{{\mathcal h}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\ci}{{\mathcal i}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cj}{{\mathcal j}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\ck}{{\mathcal k}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cl}{{\mathcal l}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cm}{{\mathcal m}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cn}{{\mathcal n}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\co}{{\mathcal o}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cp}{{\mathcal p}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cq}{{\mathcal q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\mcr}{{\mathcal r}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cs}{{\mathcal s}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\ct}{{\mathcal t}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cu}{{\mathcal u}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cv}{{\mathcal v}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\mcw}{{\mathcal w}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cx}{{\mathcal x}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cy}{{\mathcal y}}
\newcommand{\cZ}{{\mathcal Z}}
\newcommand{\cz}{{\mathcal z}}
% shakti inserted the following
% bold cals
\newcommand{\bcA}{\mbox{\boldmath $\cA$}}
\newcommand{\bcB}{\mbox{\boldmath $\cB$}}
\newcommand{\bcb}{\mbox{\boldmath $\cb$}}
\newcommand{\bcC}{\mbox{\boldmath $\cC$}}
\newcommand{\bcc}{\mbox{\boldmath $\cc$}}
\newcommand{\bcD}{\mbox{\boldmath $\cD$}}
\newcommand{\bcE}{\mbox{\boldmath $\cE$}}
\newcommand{\bcF}{\mbox{\boldmath $\cF$}}
\newcommand{\bcG}{\mbox{\boldmath $\cG$}}
\newcommand{\bcg}{\mbox{\boldmath $\cg$}}
\newcommand{\bcH}{\mbox{\boldmath $\cH$}}
\newcommand{\bcI}{\mbox{\boldmath $\cI$}}
\newcommand{\bcJ}{\mbox{\boldmath $\cJ$}}
\newcommand{\bcK}{\mbox{\boldmath $\cK$}}
\newcommand{\bcL}{\mbox{\boldmath $\cL$}}
\newcommand{\bcM}{\mbox{\boldmath $\cM$}}
\newcommand{\bcN}{\mbox{\boldmath $\cN$}}
\newcommand{\bcO}{\mbox{\boldmath $\cO$}}
\newcommand{\bcP}{\mbox{\boldmath $\cP$}}
\newcommand{\bcQ}{\mbox{\boldmath $\cQ$}}
\newcommand{\bcq}{\mbox{\boldmath $\cq$}}
\newcommand{\bcR}{\mbox{\boldmath $\cR$}}
\newcommand{\bcS}{\mbox{\boldmath $\cS$}}
\newcommand{\bcT}{\mbox{\boldmath $\cT$}}
\newcommand{\bcU}{\mbox{\boldmath $\cU$}}
\newcommand{\bcV}{\mbox{\boldmath $\cV$}}
\newcommand{\bcW}{\mbox{\boldmath $\cW$}}
\newcommand{\bmcw}{\mbox{\boldmath $\mcw$}}
\newcommand{\bcX}{\mbox{\boldmath $\cX$}}
\newcommand{\bcY}{\mbox{\boldmath $\cY$}}
\newcommand{\bcZ}{\mbox{\boldmath $\cZ$}}





% shakti: bold greek letters
\newcommand{\bgT}{\mbox{\boldmath $\Theta$}} % here for legacy reasons
\newcommand{\oalpha}{\boldsymbol{\alpha}} % here for legacy reasons
% shakti: all bold Greek letters will have the same naming conventions \bg<latex symbol name>
\newcommand{\bgalpha}{\boldsymbol{\alpha}}
\newcommand{\bgeta}{\boldsymbol{\eta}}
\newcommand{\bgTheta}{\boldsymbol{\Theta}}
\newcommand{\bgXi}{\boldsymbol{\Xi}}
\newcommand{\bglambda}{\boldsymbol{\lambda}}
\newcommand{\bgLambda}{\boldsymbol{\Lambda}}
\newcommand{\bgSigma}{\boldsymbol{\Sigma}}
\newcommand{\bgGamma}{\boldsymbol{\Gamma}}
\newcommand{\bgPhi}{\boldsymbol{\Phi}}
\newcommand{\bgDelta}{\boldsymbol{\Delta}}
\newcommand{\overbdmA}{\mbox{\boldmath $\bar{A}$}}
\newcommand{\overtau}{\mbox{$\overline{\cT}$}}
\newcommand{\tiltau}{\mbox{$\widetilde{\cT}$}}
\newcommand{\overbdmV}{\mbox{\boldmath $\bar{V}$}}

\newcommand{\overdelta}{\mbox{$\bar{\delta}$}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
%\newcommand{\balpha}{\mbox{$\bm{\alpha}$}}
\newcommand{\boalpha}{\mbox{$\overline{\balpha}$}}
\newcommand{\btalpha}{\mbox{$\widetilde{\balpha}$}}
\newcommand{\booalpha}{\mbox{$\overline{\overline{\balpha}}$}}

\newcommand{\bttalpha}{\mbox{$\widetilde{\widetilde{\boldmath \alpha}}$}}
% shakti: greek letters
\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\gd}{\delta}
\newcommand{\gk}{\kappa}
\newcommand{\gn}{\nu}

\newcommand{\sv}{\mbox{$\sigma^2_v$}}
\newcommand{\sa}{\mbox{$\sigma^2_a$}}
\newcommand{\se}{\mbox{$\sigma^2_e$}}

\newcommand{\Range}{{Range\,}}

\newcommand{\dsum}{\displaystyle\sum}
\newcommand{\disfrac}{\displaystyle\frac}
\newcommand{\dmin}{\displaystyle\min}
\newcommand{\dmax}{\displaystyle\max}

\def\adots{\mathinner{\mskip0mu\raise0pt\vbox{\kern7pt\hbox{.}}\mskip3mu
          \raise4pt\hbox{.}\mskip3mu\raise8pt\hbox{.}\mskip0mu}}
          
\newcommand{\schwa}{\raisebox{1ex}{\begin{turn}{180}e\end{turn}}}

\newcommand{\arcsinh}{\mathop\mathrm{arcsinh}\nolimits}
\newcommand{\arccosh}{\mathop\mathrm{arccosh}\nolimits}
\newcommand{\Pu}{P_{\mathrm{amb}}}

\newcommand{\bfY}{\textbf{Y}}
\newcommand{\bfF}{\textbf F}
\newcommand{\bfH}{\textbf H}
\newcommand{\bfG}{\textbf G}
\newcommand{\bfZ}{\textbf Z}
\newcommand{\bfy}{\textbf y}
\newcommand{\bfz}{\textbf z}
\newcommand{\bfs}{\textbf s}
\newcommand{\bfx}{\textbf x}
\newcommand{\bfh}{\textbf h}
\newcommand{\Nt}{{N_t}}
\newcommand{\Nr}{{N_r}}
\newcommand{\diag}{\mbox{diag}}
\newcommand{\Diag}{\mbox{Diag}}
\newcommand{\offdiag}{\mbox{offdiag}}
\newcommand{\Proj}{\mbox{Proj}}
\newcommand{\bmc}{{\boldsymbol c}}
\newcommand{\hh}{\widehat{\bfh}}
\newcommand{\Thetat}{\widetilde{\Theta}}
\newcommand{\rbar}{\overline{r}}
\newcommand{\bmW}{{\boldsymbol W}}
\newcommand{\bmV}{{\boldsymbol V}}

\newcommand{\vy}{\vettore{y}}
\newcommand{\vf}{\vettore{f}}
\newcommand{\vg}{\vettore{g}}
\newcommand{\vv}{\vettore{v}}
\newcommand{\mH}{\matrice{H}}
\newcommand{\mY}{\matrice{Y}}
\newcommand{\xh}{\widehat{x}}
\newcommand{\vfh}{\widehat{\vf}}
\newcommand{\vfhh}{\widehat{\vfh}}
\newcommand{\vgh}{\widehat{\vg}}
\newcommand{\mHh}{\widehat{\mH}}
\newcommand{\alphah}{\widehat{\alpha}}
\newcommand{\mHt}{\widetilde{\mH}}

\newcommand{\bfv}{\textbf v}
\newcommand{\bfa}{\textbf a}
\newcommand{\bfT}{\textbf T}
\newcommand{\bfR}{\textbf R}
\newcommand{\Ns}{{N_s}}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\vect}{\mbox{vec}}
\newcommand{\SNR}{\mbox{SNR}}
\newcommand{\MFB}{\mbox{MFB}}
\newcommand{\bfV}{\textbf V}
\newcommand{\bfU}{\textbf U}
\newcommand{\bfW}{\textbf W}
\newcommand{\blockdiag}{\mbox{blockdiag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bmh}{\bfh}
\newcommand{\bfu}{\textbf u}
\newcommand{\bfw}{\textbf w}
\newcommand{\ah}{\widehat{a}}
\newcommand{\bfD}{\textbf D}
\newcommand{\bfg}{\textbf g}
\newcommand{\dlim}{\displaystyle\lim}



\usepackage{bm}
\newcommand{\bmcA}{{\bm \cA}}
\newcommand{\bmtheta}{{\bm \theta}}
\newcommand{\bme}{{\bm e}}
\newcommand{\bmx}{{\bm x}}
\newcommand{\bmy}{{\bm y}}
\newcommand{\bmv}{{\bm v}}
\newcommand{\bmw}{{\bm w}}
\newcommand{\bmF}{{\bm F}}
\newcommand{\bmG}{{\bm G}}
\newcommand{\bmH}{{\bm H}}
\newcommand{\bmQ}{{\bm Q}}
\newcommand{\bmR}{{\bm R}}
\newcommand{\bmP}{{\bm P}}
\newcommand{\bmf}{{\bm f}}
\renewcommand{\bmh}{{\bm h}}
\newcommand{\bmxh}{\widehat{\bmx}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\mbE}{\mathbb{E}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mU}{\mathcal{U}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mR}{\mathcal{R}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mV}{\mathcal{V}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mRh}{\widehat{\mR}}
\newcommand{\mTh}{\widehat{\mT}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\mMt}{\widetilde{\mM}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mMh}{\widehat{\mathcal{M}}}
\newcommand{\bmzh}{\widehat{\bmz}}
\newcommand{\bmyh}{\widehat{\bmy}}
\newcommand{\bmyt}{\widetilde{\bmy}}
\newcommand{\bmxt}{\widetilde{\bmx}}
\newcommand{\bmS}{{\bm S}}
\newcommand{\bmK}{{\bm K}}
\newcommand{\bmA}{{\bm A}}
\newcommand{\bmM}{{\bm M}}
\newcommand{\bmQh}{\widehat{\bmQ}}
\newcommand{\bmFh}{\widehat{\bmF}}
\newcommand{\bmGh}{\widehat{\bmG}}
\newcommand{\bmC}{{\bf C}}
\newcommand{\bmthetah}{\widehat{\bmtheta}}
\newcommand{\bmthetat}{\widetilde{\bmtheta}}
\newcommand{\bmRh}{\widehat{\bmR}}
\newcommand{\bmHh}{\widehat{\bmH}}
\newcommand{\bmhh}{\widehat{\bmh}}
\newcommand{\bmI}{{\boldsymbol {I}}}
\newcommand{\bmD}{{\boldsymbol {D}}}
\newcommand{\bmm}{{\boldsymbol {m}}}
\newcommand{\bmo}{{\boldsymbol {o}}}
\newcommand{\bmzero}{{\bm 0}}
\newcommand{\bmp}{{\bm p}}
\newcommand{\bmn}{{\bm n}}
%\newcommand{\bmv}{{\bm v}}
\newcommand{\bma}{{\bm a}}
\newcommand{\bmph}{\widehat{\bmp}}
\newcommand{\bmU}{\bm U}
\newcommand{\bmd}{\bm d}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}

\newcommand{\thetat}{\widetilde{\theta}}
\newcommand{\thetah}{\widehat{\theta}}
\newcommand{\bGammah}{\widehat{\bGamma}}
\newcommand{\bGammat}{\widetilde{\bGamma}}
\newcommand{\CRB}{\mbox{CRB}}
\newcommand{\FIM}{\mbox{FIM}}
\newcommand{\cvec}{\mbox{vec}}
%\newcommand{\rvec}{\mbox{rvec}}
%\newcommand{\bmHb}{\overline{\bmH}}
\newcommand{\bmZero}{{\bm 0}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bmeta}{\boldsymbol{\eta}}
\newcommand{\bmkappa}{\boldsymbol{\kappa}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bmah}{\widehat{\bma}}
\newcommand{\bmdh}{\widehat{\bmd}}
\newcommand{\mbI}{\mathbb{I}}

